Raiders of the Lost Architecture: Kernels for Bayesian Optimization in Conditional Parameter Spaces

In practical Bayesian optimization, we must often search over structures with differing numbers of parameters. For instance, we may wish to search over neural network architectures with an unknown number of layers. To relate performance data gathered for different architectures, we define a new kernel for conditional parameter spaces that explicitly includes information about which parameters are relevant in a given structure. We show that this kernel improves model quality and Bayesian optimization results over several simpler baseline kernels.

==> colours.tex <==
% colorbrewer paired colours
\definecolor{lightblue}{RGB}{166,206,227}
\definecolor{darkblue}{RGB}{31,120,180}
\definecolor{lightgreen}{RGB}{178,223,138}
\definecolor{darkgreen}{RGB}{51,160,44}
\definecolor{lightred}{RGB}{251,154,153}
\definecolor{darkred}{RGB}{227,26,28}
\definecolor{lightorange}{RGB}{253,191,111}
\definecolor{darkorange}{RGB}{255,127,0}
\definecolor{lightpurple}{RGB}{202,178,214}
\definecolor{darkpurple}{RGB}{106,61,154}
\definecolor{lightyellow}{RGB}{255,255,153}
\definecolor{darkyellow}{RGB}{177,89,40}

\newcommand{\darkred}[1]{\textcolor{darkred}{{#1}}}
\newcommand{\darkblue}[1]{\textcolor{darkblue}{{#1}}}
\newcommand{\darkorange}[1]{\textcolor{darkorange}{{#1}}}
\newcommand{\darkgreen}[1]{\textcolor{darkgreen}{{#1}}}
\newcommand{\darkpurple}[1]{\textcolor{darkpurple}{{#1}}}
\newcommand{\darkyellow}[1]{\textcolor{darkyellow}{{#1}}}

% base16 solarized colours
\definecolor{b16Black}{HTML}{2D2D2D} % # Base 00 - Black
\definecolor{b16Red}{HTML}{F2777A} % # Base 08 - Red
\definecolor{b16Green}{HTML}{99CC99} % # Base 0B - Green
\definecolor{b16Yellow}{HTML}{FFCC66} % # Base 0A - Yellow
\definecolor{b16Blue}{HTML}{6699CC} % # Base 0D - Blue
\definecolor{b16Magenta}{HTML}{CC99CC} % # Base 0E - Magenta
\definecolor{b16Cyan}{HTML}{66CCCC} % # Base 0C - Cyan
\definecolor{b16White}{HTML}{D3D0C8} % # Base 05 - White
\definecolor{b16BrightBlack}{HTML}{747369} % # Base 03 - Bright Black
\definecolor{b16BrightWhite}{HTML}{F2F0EC} % # Base 07 - Bright White

% base16 eighties colours
\definecolor{b1600}{HTML}{2D2D2D}
\definecolor{b1601}{HTML}{393939}
\definecolor{b1602}{HTML}{515151}
\definecolor{b1603}{HTML}{747369}
\definecolor{b1604}{HTML}{A09F93}
\definecolor{b1605}{HTML}{D3D0C8}
\definecolor{b1606}{HTML}{E8E6DF}
\definecolor{b1607}{HTML}{F2F0EC}
\definecolor{b1608}{HTML}{F2777A}
\definecolor{b1609}{HTML}{F99157}
\definecolor{b160A}{HTML}{FFCC66}
\definecolor{b160B}{HTML}{99CC99}
\definecolor{b160C}{HTML}{66CCCC}
\definecolor{b160D}{HTML}{6699CC}
\definecolor{b160E}{HTML}{CC99CC}
\definecolor{b160F}{HTML}{D27B53}

\newcommand{\red}[1]{\textcolor{b1608}{{#1}}}
\newcommand{\blue}[1]{\textcolor{b160D}{{#1}}}
\newcommand{\orange}[1]{\textcolor{b1609}{{#1}}}
\newcommand{\green}[1]{\textcolor{b160B}{{#1}}}
\newcommand{\purple}[1]{\textcolor{b160E}{{#1}}}
\newcommand{\brown}[1]{\textcolor{b160F}{{#1}}}
\newcommand{\cyan}[1]{\textcolor{b160C}{{#1}}}
\newcommand{\yellow}[1]{\textcolor{b160A}{{#1}}}

==> figures/boxkernel.tex <==
% A simple figure to illustrate box embedding
% Jan 2014

\newcommand{\scaleamount}{0.8}
\newcommand{\anglemin}{40}
\newcommand{\angleminplusone}{41}
\newcommand{\anglemax}{150}
\newcommand{\angleone}{70}
\newcommand{\angletwo}{120}
\newcommand{\bigradius}{3.75}
\newcommand{\biggerradius}{3.3}
\newcommand{\smallradius}{0.5}
\newcommand{\xtwolabelangle}{90}
\newcommand{\belowamount}{0.2cm}
\newcommand{\belowamounttwo}{0.11cm}
\newcommand{\myell}{l}
\newcommand{\embedding}{g}

%\begin{center}
%\framebox{
\begin{tikzpicture}
[trans/.style={thick,->,shorten >=2pt,shorten <=2pt,>=stealth},scale=\scaleamount, every node/.style={transform shape}]

\tikzset{state/.style={circle,draw=black, very thick,minimum size=4em}}

\def\centerarc[#1] (#2) (#3:#4:#5)% [draw options] (center) (initial angle:final angle:radius)
{ \draw[#1] (#2) ++(#3:#5) arc (#3:#4:#5);
}
	\coordinate (x2span) at (6, 0);

	\coordinate (left) at ({\bigradius*cos(\anglemax)}, {\bigradius*sin(\anglemax)});
	\coordinate (right) at ($ (left) + (x2span) $);
	%\coordinate (right) at ({\bigradius*cos(\anglemin)}, {\bigradius*sin(\anglemin)});

	\coordinate (O1) at (-2, 0);
	\coordinate (O2) at (3, 1.25);
	
	\coordinate (left1) at ($ (left) + (O1) $);
	\coordinate (right1) at ($ (right) + (O1) $);
	\coordinate (left2) at ($ (left) + (O2) $);
	\coordinate (right2) at ($ (right) + (O2) $);
	
	% First arc
	% ==================
	
	% Draw arcs
%	\centerarc[thick] (O1) (\anglemin:\anglemax:\bigradius)
	\draw[thick] (left1) -- (right1);
%	\centerarc[thick] (O1) (\anglemin:\anglemax:\smallradius)

	\draw[fill] (left1) circle (1.5pt);
	\draw (left1) node[below = \belowamount] (l1below) {$\embedding(0, 1, \textnormal{true})$};
	
	\draw[fill] (right1) circle (1.5pt);
	\draw (right1) node[below = \belowamount] (r1below) {$\embedding(0, 0, \textnormal{true})$};

	\draw[fill] (O1) circle (1.5pt);
	\draw (O1) node[below = \belowamount] (o1below) {}
	           node[left = 0.3cm] {$\embedding(0, \cdot, \textnormal{false})$};

	%\draw (left1) -- (O1) node[above] {$\rho \pi$};
	%\draw (right1) -- (O1) node[midway, below] {$\omega$};
	
	
	% Second arc
	% ================================
	%\centerarc[thick] (O2) (\anglemin:\anglemax:\bigradius)
	%\centerarc[thick] (O2) (\anglemin:\anglemax:\smallradius)
	\draw[thick] (left2) -- (right2);

	\draw[fill] (left2) circle (1.5pt);
	
	\draw[fill] (right2) circle (1.5pt);
	\draw (right2) node[below = \belowamount] (r2below) {};
	

	\draw[fill] (O2) circle (1.5pt);
	\draw (O2) node[below = \belowamount] (o2below) {}
                   node[right] {$\embedding(1, \cdot, \textnormal{false})$};

	%\draw[dashed] (left2) -- (O2);
	%\draw[dashed] (right2) -- (O2);


	% Connect the arcs
	\draw (left1) -- (left2);
	\draw (right1) -- (right2);
	\draw[thick] (O1) -- (O2);
	
	% Draw surface
	\foreach \i in {\angleminplusone, ..., \anglemax}
	{
%		\coordinate (arca) at (\i, \i);
%		\coordinate (arca1) at ($ (arca) / 100 + (O1) $);
%		\coordinate (arca2) at ($ (arca) / 100 + (O2) $);
%		\coordinate (arcb1) at ($ (arcb) + (O1) $);
%		\coordinate (arcb2) at ($ (arcb) + (O2) $);
%		\draw[green] (arca1) -- (arca2);
%		\fill[fill=blue!40,fill opacity=0.8](arca1)--(arca2)--(arcb2)--(arcb1)--cycle;
	}

	\draw (right2) node[above] {$\embedding(1, 1, \textnormal{true})$};

	% Draw arrows showing in which direction x1 varies.
	\coordinate(x1half) at ($ (right1)!0.5!(right2) $);
	\draw (x1half) node[below = \belowamounttwo] (x1halfbelow) {$x_1$};
	\draw[trans] ($ (r1below)!0.45!(r2below) $) -- ($ (r1below)!0.3!(r2below) $);
	\draw[trans] ($ (r1below)!0.55!(r2below) $) -- ($ (r1below)!0.7!(r2below) $);

	\coordinate(x2half) at ($ (O1)!0.6!(O2) $);
	\draw (x2half) node[below = \belowamounttwo] (x2halfbelow) {$x_1$};
	\draw[trans] ($ (o1below)!0.55!(o2below) $) -- ($ (o1below)!0.4!(o2below) $);
	\draw[trans] ($ (o1below)!0.65!(o2below) $) -- ($ (o1below)!0.8!(o2below) $);

	% Draw arrows showing in which direction x2 varies.
	\coordinate(x22half) at ($ (l1below)!0.5!(r1below) $);
	\draw (x22half) node (x22halfbelow) {$x_2$};
	\draw[trans] ($ (l1below)!0.45!(r1below) $) -- ($ (l1below)!0.3!(r1below) $);
	\draw[trans] ($ (l1below)!0.55!(r1below) $) -- ($ (l1below)!0.7!(r1below) $);
\end{tikzpicture}


==> figures/semicircle.tex <==
% A simple figure to illustrate Mike and Frank's embedding
% Sept 2013

\begin{figure}
\begin{center}
  \begin{tikzpicture}

\pgfmathsetlengthmacro{\r}{3cm}
	\coordinate (O) at (0, 0);
	\coordinate (left) at ({3*cos(150)}, {3*sin(150)});

	\coordinate (right) at (\r, 0);
	\coordinate (x1) at ({3*cos(120)}, {3*sin(120)});
	\coordinate (x2) at ({3*cos(70)}, {3*sin(70)});

	% Draw big arc	
	\draw [black,thick,domain=0:150] plot ({3*cos(\x)}, {3*sin(\x)});

	\draw[fill] (left) circle (1.5pt);
	\draw (left) node[below, left] {$f(u, \textnormal{true})$};
	
	\draw[fill] (right) circle (1.5pt);
	\draw (right) node[below] {$f(\ell, \textnormal{true})$};

	\draw[fill] (O) circle (1.5pt);
	\draw (O) node[below] {$f(\cdot, \textnormal{false})$};

	\draw[fill] (x1) circle (1.5pt);
	\draw (x1) node[above, left] {$f(x_1, \textnormal{true})$};

	\draw[fill] (x2) circle (1.5pt);
	\draw (x2) node[above, right] {$f(x_2, \textnormal{true})$};
	
	% Draw little arc to denote the angle
	\draw (left) -- (O) node[above] {$\rho \pi$};
	\draw (right) -- (O) node[above] {$\rho \pi$};
	\draw [black,domain=0:150] plot ({0.5*cos(\x)}, {0.5*sin(\x)});
	
  \end{tikzpicture}
\end{center}
\caption{A demonstration of the embedding giving rise to the pseduo-metric: All points for which $\delta_i(x) =$ false are mapped to the same point.  Points for which $\delta_i(x) =$ true are mapped to a semicircle.  This embedding gives a constant distance between pairs of points which have differing values of $\delta$.  The parameter $\rho$ determines how much distance there is along the arc.}
\end{figure}



==> include/commenting.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% EDITING HELPER FUNCTIONS  %%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% NA: needs attention (rough writing whose correctness needs to be verified)
%% TBD: instructions for how to fix a gap ("Describe the propagation by ...")
%% PROBLEM: bug or missing crucial bit 

%% use \fXXX versions of these macros to put additional explanation into a footnote.  
%% The idea is that we don't want to interrupt the flow of the paper or make it 
%% impossible to read because there are a bunch of comments.

%% NA's (and TBDs, those less crucially) should be written so 
%% that they flow with the text.

\definecolor{WowColor}{rgb}{.75,0,.75}
\definecolor{SubtleColor}{rgb}{0,0,.50}

% inline
\newcommand{\NA}[1]{\textcolor{SubtleColor}{ {\tiny \bf ($\star$)} #1}}
\newcommand{\LATER}[1]{\textcolor{SubtleColor}{ {\tiny \bf ($\dagger$)} #1}}
\newcommand{\TBD}[1]{\textcolor{SubtleColor}{ {\tiny \bf (!)} #1}}
\newcommand{\PROBLEM}[1]{\textcolor{WowColor}{ {\bf (!!)} {\bf #1}}}

% as margin notes

\newcounter{margincounter}
\newcommand{\displaycounter}{{\arabic{margincounter}}}
\newcommand{\incdisplaycounter}{{\stepcounter{margincounter}\arabic{margincounter}}}

\newcommand{\fTBD}[1]{\textcolor{SubtleColor}{$\,^{(\incdisplaycounter)}$}\marginpar{\tiny\textcolor{SubtleColor}{ {\tiny $(\displaycounter)$} #1}}}

\newcommand{\fPROBLEM}[1]{\textcolor{WowColor}{$\,^{((\incdisplaycounter))}$}\marginpar{\tiny\textcolor{WowColor}{ {\bf $\mathbf{((\displaycounter))}$} {\bf #1}}}}

\newcommand{\fLATER}[1]{\textcolor{SubtleColor}{$\,^{(\incdisplaycounter\dagger)}$}\marginpar{\tiny\textcolor{SubtleColor}{ {\tiny $(\displaycounter\dagger)$} #1}}}


==> preamble.tex <==
% \renewcommand{\subparagraph}{\paragraph}
% \usepackage{include/icml2014}
\usepackage{natbib}
\usepackage{amsmath, amsthm, amssymb}
% \usepackage{pstricks}
% \usepackage{pst-tree}
%\usepackage{color}
%\usepackage{makeidx}  % allows for indexgeneration
\usepackage{bm}
%\usepackage{graphicx}
\usepackage{epsfig}
\usepackage{caption}
\usepackage{subcaption}
%\usepackage{floatrow}
\usepackage{amsmath}
\usepackage{amsfonts}
\usepackage{color}
\usepackage{array}
\usepackage{colortbl}
\usepackage{framed}
\usepackage{url}
\usepackage{booktabs}
\usepackage{multirow}
%\usepackage{sgame}
\usepackage{dsfont}
\def\sgtextcolor{black}
\def\sglinecolor{black}
%\renewcommand{\gamestretch}{2}
\usepackage{multicol}
\usepackage{lscape}
\usepackage{relsize}
\usepackage{rotating}
\usepackage{tikz}
\usetikzlibrary{calc}
% \usepackage{titlesec}


% ============== Jasper Spacing Hackery =========
%\titlespacing{\section}{0pt}{0pt}{0pt}
%\titlespacing{\subsection}{0pt}{0pt}{0pt}
%\titlespacing{\subsubsection}{0pt}{0pt}{0pt}
%\titlespacing{\paragraph}{0pt}{0pt}{10pt}
% \usepackage{enumitem}
% \setlist[itemize]{noitemsep, topsep=0pt} % Makes els 1 and 2 fit more nicely
% ===========================================

% ==============Kevin's commands ===============
%\newfloatcommand{capbtabbox}{table}[][\FBwidth]

% ============== Mike's commands ==============
\usepackage{nicefrac}
%\newcommand{\vect}[1]{\underline{\smash{#1}}}
%\newcommand{\vect}[1]{{#1}}
\renewcommand{\vec}[1]{\mathbf{#1}}
\renewcommand{\v}[1]{\vec{#1}}
\newcommand{\reals}{\mathds{R}}
\newcommand{\sX}{\mathcal{X}}
\newcommand{\sD}{\mathcal{D}}
\newcommand{\br}{}%{^{\text{\textnormal{ r}}}}
\newcommand{\cat}{^\textnormal{c}}
% ============== ==============

\newcommand{\cut}[1]{}
\newcommand{\hide}[1]{}
% \renewcommand{\blue}[1]{{\textcolor{blue}{#1}}}
%\renewcommand{\blue}[1]{#1}


\newcommand\transpose{{\textnormal{\tiny{\sf{T}}}}}
\newcommand{\hlinespace}{~\vspace*{-0.15cm}~\\\hline\\\vspace*{0.15cm}}
%\newcommand{\hlinespace}{~\vspace*{0.45cm}\\\hline\\~\vspace*{-0.9cm}}
%\newcommand{\hlinespace}{~\vspace*{0.05cm}\\\hline~\vspace*{0.5cm}}

% comment the next line to turn off notes
%\renewcommand{\note}[1]{~\\\frame{\begin{minipage}[c]{\textwidth}\vspace{2pt}\center{#1}\vspace{2pt}\end{minipage}}\vspace{3pt}\\}

\newcommand{\lnote}[1]{\note{#1}}
\newcommand{\emcite}[1]{\citet{#1}}
%\newcommand{\yrcite}[1]{\citeyear{#1}}
\newcommand{\aunpcite}[1]{\citeR{#1}}

\newcommand{\heavyrule}{\specialrule{\heavyrulewidth}{.4em}{.4em}}
\newcommand{\lightrule}{\specialrule{.03em}{.4em}{.4em}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% keep figures from going onto a page by themselves
\renewcommand{\topfraction}{0.9}
\renewcommand{\textfraction}{0.07}
\renewcommand{\floatpagefraction}{0.9}
\renewcommand{\dbltopfraction}{0.9}      % for double-column styles
\renewcommand{\dblfloatpagefraction}{0.7}   % for double-column styles

\newtheorem{thm}{Theorem}%[section]
\newtheorem{lem}[thm]{Lemma}
\newtheorem{prop}[thm]{Proposition}
\newtheorem{cor}[thm]{Corollary}
\newtheorem{obs}[thm]{Observation}

%\theoremstyle{definition}
\newtheorem{define}[thm]{Definition}
\hyphenation{ge-ne-ral-ize}

\newcommand{\Var}{\ensuremath\textnormal{Var}}
\newcommand{\indicator}{\ensuremath\mathds{I}}

%\newcommand{\fhspace}{\vspace*{0.2cm}}
%\newcommand{\newsec}{\hspace{0cm}}

% replaces tabular; takes same arguments. use \midrule for a rule, no vertical rules, and eg \cmidrule(l){2-3} as needed with \multicolumn
\newenvironment{ktabular}[1]{\sffamily\small\begin{center}\begin{tabular}[c]{#1}\toprule}{\bottomrule \end{tabular}\end{center}\normalsize\rmfamily\vspace{-5pt}}
\newcommand{\tbold}[1]{\textbf{#1}}
\newcommand{\interrowspace}{.6em}

\newcommand{\embeddingletter}{g}
\newcommand{\bo}{{\sc bo}}
\newcommand{\gp}{{\sc gp}}
\newcommand{\agp}{Arc \gp}

\usepackage{float}

==> rgb.tex <==
% colorbrewer paired colours
\definecolor{lightblue}{RGB}{166,206,227}
\definecolor{darkblue}{RGB}{31,120,180}
\definecolor{lightgreen}{RGB}{178,223,138}
\definecolor{darkgreen}{RGB}{51,160,44}
\definecolor{lightred}{RGB}{251,154,153}
\definecolor{darkred}{RGB}{227,26,28}
\definecolor{lightorange}{RGB}{253,191,111}
\definecolor{darkorange}{RGB}{255,127,0}
\definecolor{lightpurple}{RGB}{202,178,214}
\definecolor{darkpurple}{RGB}{106,61,154}
\definecolor{lightyellow}{RGB}{255,255,153}
\definecolor{darkyellow}{RGB}{177,89,40}

% base16 solarized colours
\definecolor{b16Black}{HTML}{2D2D2D} % # Base 00 - Black
\definecolor{b16Red}{HTML}{F2777A} % # Base 08 - Red
\definecolor{b16Green}{HTML}{99CC99} % # Base 0B - Green
\definecolor{b16Yellow}{HTML}{FFCC66} % # Base 0A - Yellow
\definecolor{b16Blue}{HTML}{6699CC} % # Base 0D - Blue
\definecolor{b16Magenta}{HTML}{CC99CC} % # Base 0E - Magenta
\definecolor{b16Cyan}{HTML}{66CCCC} % # Base 0C - Cyan
\definecolor{b16White}{HTML}{D3D0C8} % # Base 05 - White
\definecolor{b16BrightBlack}{HTML}{747369} % # Base 03 - Bright Black
\definecolor{b16BrightWhite}{HTML}{F2F0EC} % # Base 07 - Bright White

% base16 eighties colours
\definecolor{b1600}{HTML}{2D2D2D}
\definecolor{b1601}{HTML}{393939}
\definecolor{b1602}{HTML}{515151}
\definecolor{b1603}{HTML}{747369}
\definecolor{b1604}{HTML}{A09F93}
\definecolor{b1605}{HTML}{D3D0C8}
\definecolor{b1606}{HTML}{E8E6DF}
\definecolor{b1607}{HTML}{F2F0EC}
\definecolor{b1608}{HTML}{F2777A}
\definecolor{b1609}{HTML}{F99157}
\definecolor{b160A}{HTML}{FFCC66}
\definecolor{b160B}{HTML}{99CC99}
\definecolor{b160C}{HTML}{66CCCC}
\definecolor{b160D}{HTML}{6699CC}
\definecolor{b160E}{HTML}{CC99CC}
\definecolor{b160F}{HTML}{D27B53}

\newcommand{\red}[1]{\textcolor{b1608}{{#1}}}
\newcommand{\blue}[1]{\textcolor{b160D}{{#1}}}
\newcommand{\orange}[1]{\textcolor{b1609}{{#1}}}
\newcommand{\green}[1]{\textcolor{b160B}{{#1}}}
\newcommand{\purple}[1]{\textcolor{b160E}{{#1}}}
\newcommand{\brown}[1]{\textcolor{b160F}{{#1}}}
\newcommand{\cyan}[1]{\textcolor{b160C}{{#1}}}
\newcommand{\yellow}[1]{\textcolor{b160A}{{#1}}}

==> tables/gpml-table-old.tex <==
% --- Automatically generated by resultsToLatex4.m ---
% Exported at 20-Oct-2013 19:39:08
\begin{center}
\begin{tabular}{l | r r r r}
Method & \rotatebox{0}{ NN   }  & \rotatebox{0}{ NN   log }  & \rotatebox{0}{ NN   half }  & \rotatebox{0}{ NN   log half }  \\ \hline
Separate Linear & $\mathbf{0.968}$ & $0.886$ & $\mathbf{1.039}$ & $2.120$ \\
Separate {\sc gp} & $\mathbf{0.925}$ & $0.641$ & $\mathbf{0.860}$ & $0.848$ \\
Poor Man's embedding Linear & $\mathbf{0.905}$ & $0.763$ & $0.996$ & $0.851$ \\
Poor Man's embedding {\sc gp} & $\mathbf{0.907}$ & $0.518$ & $\mathbf{1.178}$ & $\mathbf{0.752}$ \\
Separate Hierarchical {\sc gp} & $\mathbf{0.801}$ & $0.627$ & $\mathbf{0.956}$ & $0.950$ \\
Hierarchical {\sc gp} & $\mathbf{0.801}$ & $\mathbf{0.441}$ & $\mathbf{0.993}$ & $\mathbf{0.674}$ \\
\end{tabular}
\end{center}
% End automatically generated LaTeX


==> tables/gpml-table.tex <==
% --- Automatically generated by resultsToLatex4.m ---
% Exported at 16-Jan-2014 18:46:19
\begin{center}
\begin{tabular}{l | r r r r r r}
Method & \rotatebox{0}{ NN   }  & \rotatebox{0}{ NN   log }  & \rotatebox{0}{ NN   half }  & \rotatebox{0}{ NN   log half }  & \rotatebox{0}{ concrete 500 }  & \rotatebox{0}{ housing }  \\ \hline
Separate Linear & $0.898$ & $0.874$ & $0.982$ & $\mathbf{3.482}$ & $\mathbf{ NaN}$ & $\mathbf{ NaN}$ \\
Separate {\sc gp} & $0.815$ & $0.547$ & $1.012$ & $0.753$ & $\mathbf{ NaN}$ & $\mathbf{ NaN}$ \\
Poor Man's embedding Linear & $0.882$ & $0.661$ & $0.980$ & $0.732$ & $0.403$ & $\mathbf{0.388}$ \\
Poor Man's embedding {\sc gp} & $\mathbf{0.787}$ & $\mathbf{0.498}$ & $0.819$ & $0.656$ & $\mathbf{0.164}$ & $\mathbf{0.284}$ \\
Separate Hierarchical {\sc gp} & $0.771$ & $0.554$ & $\mathbf{0.983}$ & $0.847$ & $\mathbf{ NaN}$ & $\mathbf{ NaN}$ \\
Hierarchical {\sc gp} & $0.744$ & $\mathbf{0.450}$ & $\mathbf{0.674}$ & $\mathbf{0.607}$ & $1.217$ & $\mathbf{0.411}$ \\
sep box & $\mathbf{0.687}$ & $\mathbf{0.519}$ & $\mathbf{0.753}$ & $\mathbf{0.598}$ & $\mathbf{ NaN}$ & $\mathbf{ NaN}$ \\
gp box & $\mathbf{0.621}$ & $\mathbf{0.485}$ & $\mathbf{0.675}$ & $\mathbf{0.575}$ & $0.836$ & $1.087$ \\
\end{tabular}
\end{center}
% End automatically generated LaTeX


==> tables/mcmc-table-transposed.tex <==
% --- Automatically generated by resultsToLatex4.m ---
% Exported at 20-Oct-2013 19:39:08
\begin{center}
{\small
\begin{tabular}{l | r r r r r r}
Method & Separate Linear & Separate \gp{} & Separate \agp{} & Linear & \gp{} &\agp{} \\ \hline
Original data & $0.812 \pm 0.045$ & $0.546 \pm 0.038$ & $0.535 \pm 0.030$ & $0.876 \pm 0.043$ & $0.481 \pm 0.031$ & $\mathbf{0.421 \pm 0.033}$ \\
Log outputs   & $0.737 \pm 0.049$ & $0.446 \pm 0.041$ & $0.440 \pm 0.031$ & $0.834 \pm 0.047$ & $0.401 \pm 0.028$ & $\mathbf{0.335 \pm 0.028}$ \\
\end{tabular}
}
\end{center}
% End automatically generated LaTeX

